Network-GIANT: Fully distributed Newton-type optimization via harmonic Hessian consensus

This paper considers the problem of distributed multi-agent learning, where the global aim is to minimize a sum of local objective (empirical loss) functions through local optimization and information exchange between neighbouring nodes. We introduce a Newton-type fully distributed optimization algorithm, Network-GIANT, which is based on GIANT, a Federated learning algorithm that relies on a centralized parameter server. The Network-GIANT algorithm is designed via a combination of gradient-tracking and a Newton-type iterative algorithm at each node with consensus based averaging of local gradient and Newton updates. We prove that our algorithm guarantees semi-global and exponential convergence to the exact solution over the network assuming strongly convex and smooth loss functions. We provide empirical evidence of the superior convergence performance of Network-GIANT over other state-of-art distributed learning algorithms such as Network-DANE and Newton-Raphson Consensus.

==> sections/05_numerical_analysis.tex <==
In this section we show the numerical experiments to evaluate the performance of the Network-GIANT algorithm and its comparison with other state-of-art distributed learning algorithms. We considered a distributed binary classification problem using logistic regression. Each node $i$ is considered to have $m^i$ data samples $(\bm{c}_i,\bm{y}_i) \in \mathbb{R}^d \times \{-1,+1\}$.
$$f_i(\bm{x}) = \frac{1}{m^i}\sum_{j=1}^{m^i}ln(1+e^{-y_{ij}(\bm{x}^T\bm{c}_{ij})}) + \frac{\lambda}{2}||\bm{x}||^2$$

\begin{figure*}[h]
    \centering
    \subfigure[a]{\includegraphics[width=0.24\textwidth]{figs/MNIST_NetworkGN_trainingLoss_iterations.pdf}} 
    \subfigure[b]{\includegraphics[width=0.24\textwidth]{figs/MNIST_Network_trainingLoss_time.pdf}} 
    \subfigure[c]{\includegraphics[width=0.24\textwidth]{figs/MNIST_Network_trainingLoss_bits.pdf}}
    \subfigure[e]{\includegraphics[width=0.24\textwidth]{figs/MNIST_NetworkGN_TestAccuracy.pdf}}
    \vspace{0.5cm}
    \subfigure{\includegraphics[width=0.95\textwidth]{figs/legend_network_and_centralized.pdf}}
    \caption{Convergence of network algorithms vs. multiple metrics on the MNIST dataset}
    \label{fig:MNIST_NG_vs_N}
\end{figure*}


The experiments are performed on MNIST \cite{lecun2010mnist} and Covertype \cite{dheeru2017uci} datasets. The MNIST data consists of handwritten images (28x28) of 10 digits (0 to 9) with 60000 training and 10000 test samples. The MNIST data has 784 features, we used Principal Component Analysis (PCA) to reduce the feature size to 300 and performed binary (digit 3 vs digit 7) classification. The Covertype data consists of 54 features and a label for forest cover type, 1 to 7, and has 580K data samples. We selected samples with two labels (Cover Type = 3 and Cover Type = 7) for binary classification.
We considered a network of 20 nodes and the weight matrix $\bm{P}$ is obtained using Metropolis-Hastings weights \cite{xiao2007distributed}. The same network and weight matrix have been used for all algorithms and datasets.



We compared the convergence performance of Network-GIANT with algorithms following the network learning framework like Network-DANE \cite{li2020communication} with K rounds of mixing, Jacobi(consensus) NRC \cite{varagnolo2015newton}, Newton Tracking \cite{zhang2021newton} and ESOM-K \cite{7576649} with K level of approximation. All the algorithms were performed on referenced hyper-parameter values in their respective papers.

Fig. 1 illustrates the convergence of the network algorithms with different metrics and their test performances on the MNIST dataset. Fig. 1(a) shows Training loss\footnote{Training Loss = $\frac{\frac{1}{n}\sum_{i=1}^{n}f_i(x)-f(x^*)}{f(x^*)} $}  vs. iteration performance. We have added the convergence graph of the centralized \footnote{centralized algorithms are the ones where data is not distributed} Gradient Descent(GD) and the centralized Newton Method as references.  Network-DANE with K=3 has the best convergence performance among the network algorithms followed by Netowrk-GIANT with K=2, and the Jacobi NRC performs worst among the network algorithms. The training loss vs. clock-time performance is depicted in Fig. 1(b), where the computational advantage of Network-GIANT is clearly visible as it takes the least time to converge followed by Network-DANE with K=3. In Fig. 1(c), a comparison of the communication efficiency of the network algorithms is shown based on the number of bits required to be transmitted among the nodes to achieve convergence. As depicted, Network-GIANT shares the least number of bits, making it the most communication-efficient algorithm, followed by Newton Tracking. Fig. 1(d) shows the optimality gap vs. iteration performance. Figure 1(e) displays a comparison of test accuracy. The results indicate that, apart from the Jacobi NRC algorithm, all other algorithms achieve comparable accuracy over time. Notably, Newton Tracking outperforms the other Network algorithms on the test data.

Figure 2 illustrates a comparison of the performance of various network algorithms on the Covertype dataset. The findings are comparable to those observed in the MNIST dataset, albeit with some distinctions. Specifically, Fig. 2(b) reveals that the Network-DANE algorithms take relatively longer computational time and perform worse than other algorithms in this respect. In Fig. 2(e), we see comparatively better performance of Jacobi NRC than on MNIST.




